Individual and gender inequality in computer science: A career study of cohorts from 1970 to 2000

Inequality prevails in science. Individual inequality means that most perish quickly and only a few are successful, while gender inequality implies that there are differences in achievements for women and men. Using large-scale bibliographic data and following a computational approach, we study the evolution of individual and gender inequality for cohorts from 1970 to 2000 in the whole field of computer science as it grows and becomes a team-based science. We find that individual inequality in productivity (publications) increases over a scholar's career but is historically invariant, while individual inequality in impact (citations), albeit larger, is stable across cohorts and careers. Gender inequality prevails regarding productivity, but there is no evidence for differences in impact. The Matthew Effect is shown to accumulate advantages to early achievements and to become stronger over the decades, indicating the rise of a "publish or perish" imperative. Only some authors manage to reap the benefits that publishing in teams promises. The Matthew Effect then amplifies initial differences and propagates the gender gap. Women continue to fall behind because they continue to be at a higher risk of dropping out for reasons that have nothing to do with early-career achievements or social support. Our findings suggest that mentoring programs for women to improve their social-networking skills can help to reduce gender inequality.

==> results/results_agg_citations_15_3_nodrop.tex <==
Cohort             &  0.05(0.00) &   0.05(0.00) &        0.05(0.00) &     0.04(0.00) \\
Female             &             &  -0.06(0.02) &       -0.01(0.01) &    -0.04(0.01) \\
Male               &             &   0.00(0.00) &        0.00(0.00) &     0.00(0.00) \\
Undetected         &             &   0.02(0.01) &        0.05(0.01) &     0.03(0.01) \\
Productivity       &             &              &        0.56(0.01) &     0.45(0.01) \\
Productivity (1st) &             &              &        0.34(0.00) &     0.33(0.01) \\
Impact             &             &              &        0.42(0.01) &     0.37(0.01) \\
Top source         &             &              &        0.19(0.00) &     0.05(0.00) \\
Collaboration network &          &              &                   &     0.02(0.01) \\
Senior support     &             &              &                   &     0.40(0.01) \\
Median team size   &             &              &                   &    -0.05(0.01) \\\hline
%Cohort size       &      119113 &       119113 &            119113 &         119113 \\
Intercept          &     -105.58 &      -105.66 &           -102.21 &         -77.45 \\
Mean squared error &        9.19 &         9.18 &              7.45 &           7.28 \\
Adjusted $R^2$     &        0.01 &         0.01 &              0.20 &           0.22 \\
\hline \hline


==> results/results_agg_hindex_15_3.tex <==
Start year         &  0.03(0.00) &  0.02(0.00) &   0.02(0.00) &   0.02(0.00) &   0.01(0.00) &   0.01(0.00) \\
Productivity       &            &  0.43(0.00) &   0.43(0.00) &   0.38(0.00) &   0.36(0.00) &   0.34(0.00) \\
Productivity (1st) &            &  0.15(0.00) &   0.14(0.00) &   0.14(0.00) &   0.14(0.00) &   0.13(0.00) \\
Recognition        &            &  0.03(0.00) &   0.03(0.00) &    0.00(0.00) &  -0.01(0.00) &  -0.12(0.00) \\
Female               &            &            &  -0.00(0.01) &  -0.04(0.00) &  -0.02(0.00) &   -0.00(0.00) \\
Male             &            &            &    0.00(0.00) &    0.00(0.00) &   0.01(0.00) &   0.01(0.00) \\
Undetected         &            &            &    0.00(0.00) &    0.00(0.00) &    0.00(0.00) &    0.00(0.00) \\
Social support     &            &            &             &   0.04(0.00) &   0.04(0.00) &   0.04(0.00) \\
Senior support     &            &            &             &   0.23(0.00) &   0.22(0.00) &    0.2(0.00) \\
Median team size   &            &            &             &  -0.11(0.00) &  -0.09(0.00) &  -0.09(0.00) \\
Top source          &            &            &             &             &   0.36(0.00) &   0.34(0.00) \\
Ability            &            &            &             &             &             &   0.06(0.00) \\
Ability (1st)      &            &            &             &             &             &   0.01(0.00) \\ \hline
%Cohort size        &     292443 &     292443 &      292443 &      292443 &      292443 &      292443 \\\hline 
Intercept          &     -56.42 &     -41.84 &      -41.63 &       -31.1 &      -29.27 &      -24.59 \\
Mean squared error                &       2.39 &       1.81 &        1.81 &        1.75 &        1.73 &        1.64 \\
%R2                 &       0.01 &       0.25 &        0.25 &        0.28 &        0.29 &        0.33 \\
Adjusted $R^2$        &       0.01 &       0.25 &        0.25 &        0.28 &        0.29 &        0.32 \\ \hline \hline

==> results/results_agg_hindex_15_3_nodrop.tex <==
Start year         &  0.02(0.0) &  0.02(0.0) &  0.02(0.0) &   0.02(0.0) &   0.02(0.0) &   0.01(0.0) \\
Productivity       &            &   0.3(0.0) &   0.3(0.0) &   0.24(0.0) &   0.23(0.0) &   0.22(0.0) \\
Productivity (1st) &            &  0.13(0.0) &  0.13(0.0) &   0.12(0.0) &   0.12(0.0) &   0.11(0.0) \\
Recognition        &            &  0.04(0.0) &  0.04(0.0) &   0.02(0.0) &   0.02(0.0) &  -0.04(0.0) \\
Female               &            &            &   0.0(0.0) &   -0.0(0.0) &   -0.0(0.0) &    0.0(0.0) \\
Male             &            &            &  -0.0(0.0) &    0.0(0.0) &    0.0(0.0) &    0.0(0.0) \\
Undetected         &            &            &  0.02(0.0) &    0.0(0.0) &    0.0(0.0) &    0.0(0.0) \\
Social support     &            &            &            &   0.02(0.0) &   0.02(0.0) &   0.02(0.0) \\
Senior support     &            &            &            &   0.17(0.0) &   0.17(0.0) &   0.15(0.0) \\
Median team size   &            &            &            &  -0.08(0.0) &  -0.07(0.0) &  -0.07(0.0) \\
Top source         &            &            &            &             &   0.14(0.0) &   0.13(0.0) \\
Ability            &            &            &            &             &             &   0.06(0.0) \\
Ability (1st)      &            &            &            &             &             &    0.0(0.0) \\ \hline
%Cohort size        &     119113 &     119113 &     119113 &      119113 &      119113 &      119113 \\\hline 
Intercept          &     -45.06 &     -39.01 &     -38.95 &      -30.16 &      -30.01 &      -25.95 \\
Mean Squared Error                &       0.93 &       0.78 &       0.78 &        0.74 &        0.74 &         0.7 \\
%R2                 &       0.02 &       0.18 &       0.18 &        0.22 &        0.22 &        0.26 \\
Adjusted $R^2$        &       0.02 &       0.18 &       0.18 &        0.22 &        0.22 &        0.26 \\ \hline \hline

==> results_agg_citations.tex <==
start year
&  2.15&(0.03) &   0.87&(0.02) &   0.87&(0.02) &   0.61&(0.02) &   0.61&(0.02) &  0.31&(0.02) \\
productivity
&   &       &   25.77&(0.22) &  25.77&(0.22) &   25.07&(0.2) &   25.09&(0.2) &  6.96&(0.15) \\
impact
&   &       &   13.14&(0.17) &  13.14&(0.17) &   12.5&(0.18) &  12.51&(0.18) &    0.0&(0.0) \\
\addlinespace

male
&      &       &   &  &   0.0& (0.0) &     0.0&(0.0) &     0.0&(0.0) &    0.0&(0.0) \\
female
&      &       &   &  &   0.0&(0.0) &     0.0&(0.0) &     0.0&(0.0) &    0.0&(0.0) \\
none 
&      &       &   &  &   0.33&(0.17) &   0.14&(0.12) &   0.15&(0.12) &    0.0&(0.0) \\
    \addlinespace

degree
&       &       &       &       &       &            &   -2.05&(0.08) &  -2.03&(0.08) &  0.57&(0.02) \\
coauthor hindex
&       &       &       &       &       &   &   5.02&(0.08) &   5.04&(0.08) &  2.81&(0.05) \\
    \addlinespace

top-venue

&       &       &       &       &       && &  
 &  -1.01&(0.08) &    0.0&(0.0) \\
     \addlinespace

quality
&       &       &       &       &   &&  &  &             &              &   1.55&(0.02)\\ 
\midrule
cohort size
&      \mcc{292,659} &       \mcc{292,659} &       \mcc{292,659} &       \mcc{292,659} &       \mcc{292,659} &      \mcc{292,659} \\
MSE 
&    \mcc{-34456.2} &     \mcc{-24449.7} &     \mcc{-24449.7} &     \mcc{-24264.6} &     \mcc{-24262.4} &      \mcc{-19491} \\
intercept       
&      \mcc{-4233} &     \mcc{-1754.37} &     \mcc{-1754.61} &     \mcc{-1244.81} &    \mcc{-1244.37} &     \mcc{-610.62} \\
R2
&        \mcc{0.01} &          \mcc{0.3} &          \mcc{0.3} &          \mcc{0.3} &          \mcc{0.3} &        \mcc{0.43} \\
